Coexistence in 5G: Analysis of Cross-Interference between OFDM/OQAM and Legacy Users

To optimize the use of the spectrum, it is expected that the next generation of wireless networks (5G) will enable coexistence of newly introduced services with legacy cellular networks. These new services, like Device-To-Device (D2D) communication, should require limited synchronization with the legacy cell to limit the amount of signaling overhead in the network. However, it is known that Cyclic Prefix-Orthogonal Frequency Division Multiplexing (CP-OFDM) used in Long Term Evolution-Advanced (LTE-A) is not fit for asynchronous environments. This has motivated the search for a new waveform, able to enhance coexistence with CP-OFDM. Namely, it has been widely suggested that new devices could use OFDM/Offset-Quadrature Amplitude Modulation (OFDM/OQAM) to reduce the interference they inject to legacy cellular users. However, values of interference are usually measured at the input antenna of the receiver, based on the PSD of the interfering signal. We showed in previous works that this measurement is not representative of the actual interference that is seen after the demodulation operations. Building on this finding, we provide in this paper the first exact closed forms of cross-interference between OFDM/OQAM and CP-OFDM users. Our results prove that using OFDM/OQAM only marginally reduces interference to legacy users, in contradiction with many results in the literature.

==> interference.tex <==
\subsection{Mean Interference}
The amount of interference suffered by $\mathcal{U}_1$ and $\mathcal{U}_2$ on each of their subcarriers can be estimated from (\ref{eq:i12}),(\ref{eq:i21}). In the \textit{Hom} scenario, both  $\boldsymbol{\eta}^{1\rightarrow 2}$ and $\boldsymbol{\eta}^{2\rightarrow 1}$ are obtained by replacing $\mathbf{y}$ in (\ref{eq:OFDM_demod}) with $\mathbf{x}_n[k]$ expression of (\ref{eq:OFDM_sig}). Then, $I^{1\rightarrow 2}$ and $I^{2\rightarrow 1}$ are obtained by substituting (\ref{eq:OFDM_demod}) in (\ref{eq:I12}) and (\ref{eq:I21}) respectively. These derivations lead to the following expressions of the interference caused by $\mathcal{U}_1$ (resp. $\mathcal{U}_2$) onto $\mathcal{U}_2$ (resp. $\mathcal{U}_1$):
%both $I^{1\rightarrow 2}$ and $I^{2\rightarrow 1}$ are given by replacing $\mathbf{y}$ in (\ref{eq:OFDM_demod}) by the signal expression of (\ref{eq:OFDM_sig}), and then putting (\ref{eq:OFDM_demod}) resp. in (\ref{eq:I12}) and (\ref{eq:I21}), which finally leads to
\begin{eqnarray}
I^{1\rightarrow 2}_{\textit{Hom}} &=& \sigma_{\mathbf{d}_1^2} \sum_{m \in \mathcal{L}_2, q \in \mathcal{L}_1} I^{1\rightarrow 2}_{\textit{Hom}}(q-m),\\
I^{2\rightarrow 1}_{\textit{Hom}} &=& \sigma_{\mathbf{d}_2^2} \sum_{m \in \mathcal{L}_1, q \in \mathcal{L}_2} I^{2\rightarrow 1}_{\textit{Hom}}(q-m),\vspace{-15pt}
\end{eqnarray}
where $\sigma_{\mathbf{d}_i^2}$ is the variance of $\mathbf{d}_i$. Besides, $\forall l$, $I_{\textit{Hom}}^{1\rightarrow 2}(l)$ (resp. $I_{\textit{Hom}}^{2\rightarrow 1}(l)$) represents the interference injected by the signal on the $q$-th subcarrier of $\mathcal{U}_1$ (resp. $\mathcal{U}_2$) onto the $m$-th subcarrier $m$ of (resp. $\mathcal{U}_1$) where $l = q-m$ is called the spectral distance. In \textit{Hom} scenario, $\forall l, I_{\textit{Hom}}^{1\rightarrow 2}(l) = I_{\textit{Hom}}^{2\rightarrow 1}(l)$, and Mejdahdi \textit{et. al.} have derived in \cite{Medjahdi2010a} a closed-form of the interference $I_{\textit{Hom}}^{1\rightarrow 2}(l)$ and tabulated its values in so-called "Mean Interference Tables".

In \textit{Het} scenario, the expression of $\boldsymbol{\eta}^{1\rightarrow 2}$ (resp. $\boldsymbol{\eta}^{2\rightarrow 1}$) is obtained by replacing $\mathbf{y}$ in (\ref{eq:OFDM_demod}) (resp. (\ref{eq:FBMCmod})) with the expression of $\mathbf{x}_n[k]$ in (\ref{eq:FBMC_sig}) (resp. (\ref{eq:OFDM_sig})). Then, values of $I^{1\rightarrow 2}$ (resp. $I^{2\rightarrow 1}$) are finally rated by substituting the resulting expression in (\ref{eq:I12}) (resp. (\ref{eq:I21})).
%$I_{\textit{Het}}^{1\rightarrow 2}$ (resp. $I_{\textit{Het}}^{2\rightarrow 1}$) is obtained by replacing $\mathbf{y}$ in (\ref{eq:OFDM_demod}) (resp. (\ref{eq:FBMCmod})) by the expression of (\ref{eq:FBMC_sig}) (resp. (\ref{eq:OFDM_sig})), and putting the resulting expression in (\ref{eq:I12}) (resp. (\ref{eq:I21})). 
After several derivation steps, we get, as in the \textit{Hom} scenario,\vspace{-8pt}
\begin{eqnarray}
I^{1\rightarrow 2}_{\textit{Het}} &=& \sigma_{\mathbf{d}_1^2} \sum_{m \in \mathcal{L}_2, q \in \mathcal{L}_1} I^{1\rightarrow 2}_{\textit{Het}}(q-m),\label{eq:I12het}\\
I^{2\rightarrow 1}_{\textit{Het}} &=& \sigma_{\mathbf{d}_2^2} \sum_{m \in \mathcal{L}_1, q \in \mathcal{L}_2} I^{2\rightarrow 1}_{\textit{Het}}(q-m).\label{eq:I21het}
\end{eqnarray}
Getting mathematical closed-forms of $I^{1\rightarrow 2}_{\textit{Het}}(l)$ and $I^{2\rightarrow 1}_{\textit{Het}}(l)$ is challenging, which is why, for sake of simplicity, most studies of mutual interference in heterogeneous scenarios are based on the PSD-based model \cite{weiss04, Xu2008, shaat2010computationally,  skrzypczak2012ofdm}.

\subsection{PSD-based Interference Modeling}

\begin{figure}
	\vspace{-10pt}
	\centering
	\subfloat{\label{fig:PSD_OFDM}	\includegraphics[width=\linewidth]{PSD_model_OFDM.eps}}
	\hspace{5pt}
	\subfloat{\label{fig:PSD_OQAM}	\includegraphics[width=\linewidth]{PSD_model_PHYDYAS.eps}}
	\caption{Modeling of injected interference with the PSD-based model for CP-OFDM (top) and OFDM/OQAM with PHYDYAS filter (bottom). The values of interference injected by subcarrier $0$ on a subcarrier at a spectral distance of $l=1$ correspond to the integration of the PSD from $0.5\ \Delta F$ to $1.5\ \Delta F$.}
	\label{fig:PSD_model}
	\vspace{-10pt}
\end{figure}

The PSD-based model consists in computing the leakage caused by users onto each other by integrating the PSD of the interfering signal on the band that suffers from the interference. Therefore, in the \textit{Het} scenario, according to the PSD-based model, (\ref{eq:I12het}) and (\ref{eq:I21het}) are obtained by computing
\begin{eqnarray}
I_\textit{Het}^{1\rightarrow 2}(l) &=& \int\limits_{l-1/2\Delta F}^{l+1/2\Delta F}\Phi_\text{CP-OFDM}(f) df,\label{eq:PSD_mod1}\\
I_\textit{Het}^{2\rightarrow 1}(l) &=& \int\limits_{l-1/2\Delta F}^{l+1/2\Delta F}\Phi_\text{PHYDIAS}(f) df,\label{eq:PSD_mod}
\end{eqnarray}
where $\Phi_\text{CP-OFDM}$ (resp. $\Phi_\text{PHYDIAS}$ ) is the PSD of the CP-OFDM signal (resp. of OFDM/OQAM with PHYDIAS filter).
A graphical view of (\ref{eq:PSD_mod1}) and (\ref{eq:PSD_mod}) is presented in Fig.~\ref{fig:PSD_model}. It can be seen than values of interference rated with the PSD-based model are not symmetrical. As a matter of fact, because the side-lobes of $\Phi_\text{CP-OFDM}$ are much higher than those of $\Phi_\text{PHYDIAS}$, the PSD-based model will give $I_\textit{Het}^{1\rightarrow 2} \gg I_\textit{Het}^{2\rightarrow 1}$. Therefore, according to the PSD-based model, the CP-OFDM incumbent $\mathcal{U}_1$ interferes more onto the OFDM/OQAM secondary $\mathcal{U}_2$ than the opposite.

Besides, because the PSD-based model only rates the power of injected interference, it is challenging to map the obtained values of interference to higher level metrics, e.g. Bit Error Rate (BER). The only possibility offered by the PSD-based model is to approximate the statistics of heterogeneous interference as a white Gaussian noise the variance of which is given by (\ref{eq:PSD_mod}), i.e 
\begin{equation}
\boldsymbol{\eta}_m^{2\rightarrow 1} \sim \mathcal{N}(0,\sum_{q\in \mathcal{L_1}}I_\textit{Het}^{2\rightarrow 1}(q-m)).
\end{equation}
Then, classical expressions of transmission performance under white Gaussian noise in \cite{ProakisAWGN} can be applied.
%Besides, in analysis based on the PSD-based model, classical expressions of transmission performance under white Gaussian noise in \cite{ProakisAWGN} are used \cite{shaat2010computationally}. This shows that these studies model heterogeneous interference as a white Gaussian noise \cite{shaat2010computationally} the variance of which is given by (\ref{eq:PSD_mod}), e.g, 

\subsection{Discussing the suitability of the PSD-based model}
\label{sec:discuss}
\begin{figure}
		\vspace{-20pt}
	\includegraphics[width=\linewidth]{exp2.eps}
\vspace{-50pt}
	\caption{Demodulation operations at the CP-OFDM receiver with an interfering OFDM/OQAM signal. The well-shaped PHYDYAS filter is cut in small non-contiguous parts on which FFT operations are performed.}
	\vspace{-10pt}
	\label{fig:explanation}
\end{figure}

The main pitfall of the PSD-based model lies in the fact that it does not take into account the time window of the receiver. However, this is of paramount importance as the incumbent only considers a time window with a specific width based on its own parameters. To illustrate this, Fig.~\ref{fig:explanation} shows the demodulation operations that are performed by the CP-OFDM incumbent with an interfering secondary OFDM/OQAM signal. Though the PHYDYAS filter is well spectrally localized, it has a length of  $L_\text{PHYDYAS} = KM$ samples. However, the CP-OFDM receiver window is of length $L_\text{CP-OFDM} = M$ samples. Therefore, as plotted in Fig.~\ref{fig:explanation}, the CP-OFDM incumbent demodulator performs Fast Fourier Transform (FFT) on a time window which is much shorter than the length of the prototype filter of OFDM/OQAM. In turn, the signal suffers from discontinuities that produce projections on the whole incumbent spectrum. 

Moreover, Fig.~\ref{fig:PSD_model} shows that the PSD based model consists in multiplying the interfering signal by a rectangular window in the frequency domain. In the time domain, this corresponds to filtering the interfering signal through an infinite sinc filter. Therefore, the PSD-based model does not reflect the actual demodulation operations that are processed at the CP-OFDM receiver that suffers from interference. 

Besides, Fig.~\ref{fig:explanation} shows that the prototype filter of OFDM/OQAM spans multiple time windows of the CP-OFDM incumbent receiver. Then, one OFDM/OQAM symbol interferes on several subsequent CP-OFDM symbols. This shows that the elements of $\boldsymbol{\eta}^{2\rightarrow 1}$ cannot be considered independent. Therefore, though Gaussian, the heterogeneous interference between the two users in \textit{Het} scenario is not white, but colored. 
%We recall that, in this paper, we aim to rate the inter-user interference caused by the coexistence between CP-OFDM based $\mathcal{U}_1$ and OFDM/OQAM based $\mathcal{U}_2$ as defined in (\ref{eq:interfExpression}). The classical way to compute the leakage is to integrate the Power Spectral Density (PSD) of the interfering signal on the band that suffers from the interference \cite{weiss04, shaat2010computationally}, which is hereafter referred to as the PSD-based model.





%According to the PSD-based model, the interfering signal can be expressed as a sum of interfering signals coming from each subcarrier of the interfering user as 
%\begin{equation}
%\mathbf{i}_n^{j\rightarrow i}[m] = \sum_{q \in \mathcal{L}_j} \mathbf{i}_{n,q}^{j\rightarrow i}[m], 
%\end{equation}
%where each signal $\mathbf{i}_{n,q}^{j\rightarrow i}[m]$ is modeled as a white Gaussian process of variance $I_{i\rightarrow j,q}^m$. It is worth noting that this term only depends on the difference $l = m-q$ called spectral distance. Then, the value of $I_{i\rightarrow j}(l)$ is obtained by integrating the PSD of the interfering signal as \cite{weiss04}
%\begin{equation}
%\label{eq:PSD_model}
%I_{i\rightarrow j}(l) = \int\limits_{l-1/2\Delta F}^{l+1/2\Delta F}\Phi_i(f) df,
%\end{equation}
%The application of the PSD-based model to both CP-OFDM and OFDM/OQAM system for spectral distance $l = 1$ is represented in Fig.~\ref{fig:PSD_model}.
%
%Then, the total interference power is obtained by the summation of $I_{i\rightarrow j}(l)$ as 
%\begin{equation}
%I_{i\rightarrow j} = \sum_{m \in \mathcal{L}_i, q \in \mathcal{L}_j} I_{i\rightarrow j}(q-m).
%\end{equation}
%
%Several observations can be made from this definition of interference. First, the computed interference value only depends on the shape of the transmitted interfering signal, before demodulation by the receiver. Therefore, in a heterogeneous context, the computed inter-user interference is not symmetrical. Indeed, in the scenario under study, it gives:
%\begin{align}
%I_{1\rightarrow 2}(l) &= \int\limits_{l-1/2\Delta F}^{l+1/2\Delta F}\Phi_\text{CP-OFDM}(f) df\\
%I_{2\rightarrow 1}(l) &= \int\limits_{l-1/2\Delta F}^{l+1/2\Delta F}\Phi_\text{Phydias}(f) df
%\end{align}
%Therefore, because of the better shape of the Phydias PSD, the PSD-based model predicts that $\mathcal{U}_1$ interferes more onto $\mathcal{U}_2$ than $\mathcal{U}_2$ onto $\mathcal{U}_1$, as shown in Fig.~\ref{fig:PSD_model}
%
%Besides, considering a generic interfering signal $y(t)$ of Fourier transform $\mathcal{Y}$, and naming $\Pi_l(f)$ the frequency rectangular function equal to zero everywhere except for $l-1/2\Delta F \leq l+1/2\Delta F$ , the PSD based model gives
%\begin{align}
%\label{eq:PSD_modelb}
%I(l) &= \int\limits_{-\infty}^{+\infty} \left|\mathcal{Y}(f)\Pi_l(f)\right|^2 df \\
%&= \int\limits_{-\infty}^{+\infty} \left|\mathcal{F}\left\{y(t)*\left(\Delta F \text{sinc}(\pi\Delta F t)e^{jl\Delta Ft}\right)\right\}\right|^2 df.
%\end{align}
%
%Therefore, using the PSD based model equates to considering that the interfering signal $y$ is filtered through an infinite sinc filter, regardless of the actual receiver suffering from interference. In fact, the PSD based model is an approximation which consists in considering interference power at the antenna of the receiver and neglects all the demodulation operations performed by the receiver. Though it may give good approximations in certain scenarios, we explain why it is not suitable in heterogeneous coexistence context in the following subsection.
%
%\subsection{Instantaneous interference approach}
%\begin{figure}
%	\includegraphics[width=\linewidth]{OFDMdemodOfFBMC.eps}
%	\caption{Demodulation of interfering OFDM/OQAM signal at the CP-OFDM receiver.}
%	\label{fig:explanation}
%\end{figure}
%
%To overcome the aforementioned drawbacks of the PSD based model, Medjahdi \textit{et. al.} have developed the concept of "instantaneous interference tables", which consists in rigorously evaluating (\ref{eq:interfExpression}), and analytical expressions for asynchronous interference between homogeneous users using either CP-OFDM of OFDM/OQAM have been derived in \cite{Medjahdi2010a}.
%
%Following this approach in the context of our paper, the inter-user interference is obtained by analyzing the reception of a OFDM/OQAM signal by a CP-OFDM receiver. This operation is represented in Fig.~\ref{fig:explanation}. On this figure, it appears clearly why the PSD-based model is not suitable in this study: the CP-OFDM receiver cuts the incoming OFDM/OQAM signal in multiple non-contiguous small parts before processing a Fast Fourier Transform (FFT) on each part, which incurs projections on the whole band. Doing so, the good spectral properties of the Phydias prototype filter are lost, and the interference seen by the CP-OFDM receiver after demodulation is much higher than what is obtained by the PSD-based model.
%
%Besides, in the scenario under study, it appears that the inter-user interference cannot be modeled as white Gaussian signal. Indeed, Fig.~{\ref{fig:explanation}} shows that one OFDM/OQAM symbol interferes onto subsequent CP-OFDM symbols, which correlates interference seen by the CP-OFDM receiver. Because the interfering link is symmetrical between the CP-OFDM and OFDM/OQAM users, this is also true concerning the interference seen by the OFDM/OQAM receiver, as one CP-OFDM symbol affects multiple subsequent OFDM/OQAM symbols. Therefore, the inter-user interference, though Gaussian, is not white, but colored.
%
%Building on these observations, we compare in the following section the interference values that are obtained by empirical estimation of (\ref{eq:interfExpression})  and those computed with the PSD-based model.



